UniPar: A Unified LLM-Based Framework for Parallel and Accelerated Code Translation in HPC

Translating programs between various parallel programming languages is an important problem in the high-performance computing (HPC) community. Existing tools for this problem are either too narrow in scope and/or outdated. Recent explosive growth in the popularity of large language models (LLMs) and their ability to generate and translate code offers a potential alternative approach. Toward that end, we first need to systematically evaluate the ability of LLMs to translate between parallel languages. In this work, we introduce UniPar, a systematic evaluation framework for LLM-based parallel code translation. Specifically, in this work, we target translations between serial code, CUDA, and OpenMP. Our goal is to assess how well current instruction-tuned LLMs -- specifically GPT-4o-mini and LLaMA-3.3-70B-Instruct -- can be used out of the box or enhanced through known strategies. We evaluated four major usage modes: hyperparameter optimization for decoding, zero- and few-shot prompting, supervised fine-tuning, and iterative feedback through compiler-based repair. As a part of the evaluation, we construct a new dataset called PARATRANS, covering both serial-to-parallel translation and cross-paradigm transformations. Our findings reveal that while off-the-shelf models struggle under the default settings (e.g., GPT-4o-mini achieves only 46% compilation and 15% functional correctness), our UniPar methodology -- combining fine-tuning, hyperparameter tuning, and compiler-guided repair -- improves performance by up to 2X (69% compilation and 33% correctness). We believe that our findings will provide useful insights for researchers to further improve LLMs for the parallel language translation problem. UniPar source code and PARATRANS dataset are available at our GitHub repository https://github.com/Scientific-Computing-Lab/UniPar_AI.

==> to_p_comparision.tex <==
\begin{figure}[!tbp]
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=2 by 1,
        % bar width=0.12cm,
        horizontal sep=1.2cm
    },
    ybar,
    % bar width=0.12cm,
    width=0.25\textwidth,
    height=4.2cm,
    enlarge x limits={abs=0.4cm},
    symbolic x coords={LLaMA (Base), GPT-4o-mini (Base), LLaMA (FT)},
    nodes near coords,
every node near coord/.append style={font=\scriptsize, rotate=90, anchor=west},
    xtick=data,
    xticklabel style={rotate=22, anchor=east, font=\small},
    ymin=0, ymax=1,
    % grid=both,
    ymajorgrids=true,
    grid style=dashed,
    legend style={at={(1.1,-0.7)}, anchor=north, legend columns=-1, draw=none, fill=none},
    xlabel style={font=\small},
]

% First plot
\nextgroupplot[
    ylabel={Compilation Rate},
    xlabel={Questioner Model},
    bar width=0.12cm,
    % title={Compilation Rate},
]
\addplot+[fill=blue!70] coordinates {(LLaMA (FT),0.53) (LLaMA (Base),0.495) (GPT-4o-mini (Base),0.46)};

\addplot+[fill=red!70] coordinates {(LLaMA (FT),0.695) (LLaMA (Base),0.735) (GPT-4o-mini (Base),0.69)};

\addlegendentry{Without agent}
\addlegendentry{With agent}
\end{groupplot}
\end{tikzpicture}

% \caption{Figure shows the comparison of compilation and validation rates with and without agents. Agentic pipeline delivered significant improvement in both the compilation and validation rates. Although the finetuned model is less affected, it maintains the lead in terms of valid codes.}
\caption{
\textbf{Overall Impact of the Agentic Pipeline Across Different Questioner Models.}
Compilation and validation rates for various Questioner models with and without the agentic pipeline (Compilation and Execution agents). Incorporating Compilation and Execution agents leads to a substantial improvement in both metrics, especially for base models. While the fine-tuned model shows smaller gains, it consistently achieves the highest overall validation rate.
}

\label{fig:agent_comp_val}
\end{figure}
